Energy-optimal Design and Control of Electric Powertrains under Motor Thermal Constraints

This paper presents a modeling and optimization framework to minimize the energy consumption of a fully electric powertrain by optimizing its design and control strategies whilst explicitly accounting for the thermal behavior of the Electric Motor (EM). Specifically, we first derive convex models of the powertrain components, including the battery, the EM, the transmission and a Lumped Parameter Thermal Network (LPTN) capturing the thermal dynamics of the EM. Second, we frame the optimal control problem in time domain, and devise a two-step algorithm to accelerate convergence and efficiently solve the resulting convex problem via nonlinear programming. Subsequently, we present a case study for a compact family car, optimize its transmission design and operation jointly with the regenerative braking and EM cooling control strategies for a finite number of motors and transmission technologies. We validate our proposed models using the high-fidelity simulation software Motor-CAD, showing that the LPTN quite accurately captures the thermal dynamics of the EM, and that the permanent magnets' temperature is the limiting factor during extended driving. Furthermore, our results reveal that powertrains equipped with a continuously variable transmission (CVT) result into a lower energy consumption than with a fixed-gear transmission (FGT), as a CVT can lower the EM losses, resulting in lower EM temperatures. Finally, our results emphasize the significance of considering the thermal behavior when designing an EM and the potential offered by CVTs in terms of downsizing.

==> chapters/formula.tex <==
\section{formula}\label{sec:formula}

OBJECTIVE:
\begin{small}
	\begin{equation*}
		J = - E_{\mathrm{b}}(\mathrm{T}) = \int_{0}^{\mathrm{T}} P_{\mathrm{int}}~dt
	\end{equation*}
\end{small}
 
VEHICLE DYNAMICS AND TRANSMISSION:
\begin{small}
	\begin{equation*}
		\begin{aligned}
			P_{\mathrm{fd}}(t) &= P_{\mathrm{req}}(t) + P_{\mathrm{brk}}(t) \\
			P_{\mathrm{brk}}(t) &\geq 0
		\end{aligned}
	\end{equation*}
\end{small}

\begin{small}
	\begin{equation*}
		\begin{aligned}
			P_{\mathrm{req}}(t) =  v(t) \cdot \Big( \frac{1}{2} \cdot &\rho \cdot c_{\mathrm{d}} \cdot A_{\mathrm{f}} \cdot v(t)^2 +\\  &m_\mathrm{v}  \big(g \cdot c_{\mathrm{r}} \cdot cos(\alpha(t)) + g \cdot sin(\alpha(t)) + a(t) \big) \Big) 
		\end{aligned}
	\end{equation*}
\end{small}

\begin{small}
	\begin{equation*}
		\omega_{\mathrm{mot}}(t) = \gamma \cdot \gamma_{\mathrm{fd}} \cdot \frac{v(t)}{r_{\mathrm{w}}} 
	\end{equation*}
\end{small}

\begin{equation*}
	P_\mathrm{mot} (t) = 
	\left\{
	\begin{aligned}
		P_\mathrm{fd}(t) \cdot \eta_\mathrm{fgt}^{-sign(P_\mathrm{fd}(t))} \text{~~if FGT,} \\
		P_\mathrm{fd}(t) \cdot \eta_\mathrm{cvt}^{-sign(P_\mathrm{fd}(t))} \text{~~if CVT}
	\end{aligned}
	\right.
\end{equation*}


\begin{equation*}
	\gamma(t) 
	\left\{
	\begin{aligned}
		& =   &{\gamma_{\mathrm{1}}} & \text{~~if FGT,} \\
		& \in & [\gamma_{\mathrm{min}}, \gamma_{\mathrm{max}}] & \text{~~if CVT} \\
	\end{aligned}
	\right.
\end{equation*}

MASS MODELS:
\begin{equation*}
	\begin{aligned}
		m_{\mathrm{v}}   &= m_{\mathrm{0}} + m_{\mathrm{m}} \\
		m_{\mathrm{m}}   &= \bar{m}_{\mathrm{m}} \cdot s_{\mathrm{m}} \\
		s_{\mathrm{m}}^3 &= \frac{T_\mathrm{m}}{\bar{T}_\mathrm{m}} \\
	\end{aligned}
\end{equation*}

ELECTRIC MOTOR:\\
\begin{equation*}
	\begin{aligned}
		x_\mathrm{sft}(t) &= \begin{bmatrix}
			1 & \omega_{\mathrm{m}}(t)
		\end{bmatrix}^\top \\
		P_\mathrm{sft}(t) &= a_\mathrm{sft} \cdot x_\mathrm{sft}(t) 
	\end{aligned}
\end{equation*}

\begin{equation*}
	\begin{aligned}
		P_\mathrm{req} & < 0, & &\\
		& P_\mathrm{i}  &= x_\mathrm{i}(t)^\top~Q_\mathrm{i}~x_\mathrm{i}(t) &\\
		& \mathrm{i}    &= \mathrm{rtr, mgt, str, wdg} &\\ 			
		& x_\mathrm{i}(t) &= \begin{bmatrix}
			1 & \omega_{\mathrm{m}}(t) & P_{\mathrm{m}}(t) & \omega_{\mathrm{m}}(t)^2 & P_{\mathrm{m}}(t)^2 & \omega_{\mathrm{m}}(t) \cdot P_{\mathrm{m}}(t) \end{bmatrix} &\\
	\end{aligned}
\end{equation*}


\begin{small}
	\begin{equation*}
		P_\mathrm{i} = x_\mathrm{i}(t)^\mathrm{T}~Q_\mathrm{i}~x_\mathrm{i}(t)
	\end{equation*}
\end{small} 



\begin{small}
	$ x_\mathrm{rt,mg,st,wd}(t) = \begin{bmatrix}
		1 & \omega_{\mathrm{m}}(t) & P_{\mathrm{m}}(t) & \omega_{\mathrm{m}}(t)^2 & P_{\mathrm{m}}(t)^2 & \omega_{\mathrm{m}}(t) \cdot P_{\mathrm{m}}(t)
	\end{bmatrix}^\top $
\end{small}


$P_\mathrm{mot} < 0$,
\begin{small}
	$ x_\mathrm{sft}(t) = \begin{bmatrix}
		1 & \omega_{\mathrm{m}}(t)
	\end{bmatrix}^\top $
\end{small}


.

==> chapters/methodology.tex <==
\section{Methodology}\label{sec:methodology}
In this section, we present a framework based on convex optimization to optimize the design and control strategies of the electric vehicle powertrain. First, we define the optimization objective and frame the optimal control problem in the time domain. Second, we introduce the convex quasi-static models of all the powertrain components, including the transmission and battery. The state-of-the-art temperature-dependent motor loss models and thermal models are presented in Sections~\ref{sec:methodology_motor} and~\ref{sec:methodology_thermal}, respectively. Finally, we summarize the optimization problem and highlight some key features of the proposed framework.

% \mkmargin{The lower level uses convex optimization techniques while the upper levels uses grid search which when combined gives globally optimal results.}{rewrite.} 

The full-electric powertrain shown in Fig.~\ref{fig:Topology} consists of a battery that converts chemical energy to electrical energy. The inverter-motor assembly, in turn, converts it into mechanical energy, which is transferred from the motor shaft to the wheels through a gearbox and a final drive. We consider two gearboxes: an FGT and a CVT. The losses in the inverter, motor and transmission generate heat which is continuously removed from the powertrain to prevent any damage to the vehicle via a thermal circuit consisting of a radiator, fan and a coolant. The coolant transfers the thermal energy from different components to the radiator-fan assembly, which releases the heat into the atmosphere. 
\mkmargin{An electric motor is capable of recuperating a part of energy when the vehicle is decelerating which is otherwise lost to friction. The recuperation process induces losses in the motor which increases the temperature of its components.}{Explain significance of Pbrk.}
The input variables to the optimal control problem with a CVT are the mechanical brake force $P_\mathrm{brk}(t)$ and the gear ratio $\gamma(t)$. For an FGT, the only input variable is $P_\mathrm{brk}(t)$, whereas the gear ratio $\gamma$ is a design variable. The state variables are the amount of battery energy used since the start of the driving cycle $E_\mathrm{b}$, and the components' temperatures: the shaft's temperature $\vartheta_\mathrm{sft}$, the rotor's temperature $\vartheta_\mathrm{rtr}$, the permanent magnets' temperature $\vartheta_\mathrm{mgt}$, the stator's temperature $\vartheta_\mathrm{str}$, the windings' temperature $\vartheta_\mathrm{wdg}$, and the end-windings' temperature $\vartheta_\mathrm{ewdg}$. The optimal control problem will be discussed in detail below.

\subsection{Objective}\label{sec:methodology_objective}
Our objective is to minimize the internal energy consumption of the battery over a given drive cycle:
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:objective}
		J = \Delta E_{\mathrm{b}},
	\end{equation}
\end{small}%
\endgroup
where $\Delta E_{\mathrm{b}}$ is the difference in battery state of energy defined as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:DeltaEb}
		\Delta E_{\mathrm{b}} = E_{\mathrm{b}}(0) - E_{\mathrm{b}}(\mathrm{T}),
	\end{equation}
\end{small}%
\endgroup
and $E_{\mathrm{b}}(0)$ and $E_{\mathrm{b}}(\mathrm{T})$ denote the battery state of energy at the start and end of the drive cycle, respectively.

%$P_{\mathrm{int}}$ is the internal battery power. 



\subsection{Vehicle Dynamics and Transmission}\label{sec:methodology_vehicle}
In this section, we model the vehicle and the transmission in a quasi-static manner in line with the current practices~\cite{GuzzellaSciarretta2007}. In this regard, we present a convex model of the logitudinal vehicle dynamics in the time domain. To improve readability, we exclude time dependence whenever it is clear from the context. Firstly, the power equilibrium at the wheels is given as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Power_Balance_FD}
%		P_{\mathrm{fd}}(t) = P_{\mathrm{req}}(t) + P_{\mathrm{brk}}(t),
		P_{\mathrm{fd}} = P_{\mathrm{req}} + P_{\mathrm{brk}},
	\end{equation}
\end{small}%
\endgroup
\noindent where $P_{\mathrm{fd}}$ is the final drive power, $P_{\mathrm{req}}$ is the power required at the wheels and $P_{\mathrm{brk}}$ is the mechanical brake power required. As mentioned above, $P_{\mathrm{brk}}$ is an input variable, and it controls the amount of regenerative braking to maintain EM temperatures within their limits. Additionally, we constrain the brake power according to
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Pbrk>0}
%		P_{\mathrm{brk}}(t) \geq 0.
		P_{\mathrm{brk}} \geq 0.
	\end{equation}
\end{small}%
\endgroup
\noindent $P_{\mathrm{req}}$ is a combination of aerodynamic drag, rolling resistance, gravitational force and vehicle inertia. We compute $P_{\mathrm{req}}$ for a given drive cycle with a velocity $v(t)$, an acceleration $a(t)$, and a road gradient $\alpha(t)$ with
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Power_Required}
		\begin{aligned}
%			P_{\mathrm{req}}(t) =  v(t) \cdot & \Big( \frac{1}{2} \cdot \rho_{\mathrm{a}} \cdot c_{\mathrm{d}} \cdot A_{\mathrm{f}} \cdot v(t)^2 +\\  &m_\mathrm{v}  \big(g \cdot c_{\mathrm{r}} \cdot cos(\alpha(t)) + g \cdot sin(\alpha(t)) + a(t) \big) \Big),
			P_{\mathrm{req}}\big(v(t),\alpha(t),&a(t)\big) = v(t) \cdot \Big( \frac{1}{2} \cdot \rho_{\mathrm{a}} \cdot c_{\mathrm{d}} \cdot A_{\mathrm{f}} \cdot v(t)^2 + \\  &m_\mathrm{v}  \big(g \cdot c_{\mathrm{r}} \cdot \cos(\alpha(t)) + g \cdot \sin(\alpha(t)) + a(t) \big) \Big),
		\end{aligned}
	\end{equation}
\end{small}%
\endgroup
where $m_\mathrm{v}$ is the total mass of the vehicle, $c_{\mathrm{d}}$ is the vehicle's drag coefficient, $A_{\mathrm{f}}$ is the frontal area of the vehicle, $c_{\mathrm{r}}$ is the road friction coefficient, $\rho_{\mathrm{a}}$ is the air density and $g$ is the Earth's gravitational constant. We assume a constant final drive and transmission efficiency, $\eta_\mathrm{fd}$ and $\eta_\mathrm{gb}$, respectively. Therefore, the power at the motor shaft $P_\mathrm{m}$ is given by
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:FD-MOT_Power}
	%	P_\mathrm{mot} (t) = 
	%	\begin{cases}
	%		P_\mathrm{fd}(t) \cdot \eta_\mathrm{fgt}^{-sign(P_\mathrm{fd}(t))} & \text{~~if FGT,} \\
	%		P_\mathrm{fd}(t) \cdot \eta_\mathrm{cvt}^{-sign(P_\mathrm{fd}(t))} & \text{~~if CVT,}
	%	\end{cases}
		P_\mathrm{m} = 
		\begin{cases}
			\dfrac{1}{\eta_\mathrm{gb} \cdot \eta_\mathrm{fd}} \cdot P_\mathrm{fd} & \text{~~if~~} P_\mathrm{fd} \geq 0 \\
			\eta_\mathrm{gb} \cdot \eta_\mathrm{fd} \cdot r_\mathrm{b} \cdot P_\mathrm{fd} & \text{~~if~~} P_\mathrm{fd} < 0. \\
		\end{cases}
	\end{equation}
\end{small}%
\endgroup
%\mkmargin{The transmission efficiencies for FGT and CVT are}{In same equation?}
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks 
%\begin{small}
%	\begin{equation}
%		\label{eq:GB_Efficiency}
%		\eta_\mathrm{gb} = 
%		\begin{cases}
%			\eta_\mathrm{fgt} & \text{~~if  FGT,} \\
%			\eta_\mathrm{cvt} & \text{~~if  CVT,}
%		\end{cases}
%	\end{equation}
%\end{small}
%\endgroup
\mkmargin{where $\eta_\mathrm{gb} = \eta_\mathrm{fgt}$ and $\eta_\mathrm{gb} = \eta_\mathrm{cvt}$ are efficiencies of FGT and CVT, respectively}{rewrite?}, and $r_\mathrm{b}$ is the regenerative braking fraction. %To retain convexity we relax Eq.~\ref{eq:FD-MOT_Power} to
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks 
%\begin{small}
%	\begin{equation}
%	\label{eq:FD_MOT_Power_Relaxed}
%		%	P_\mathrm{mot} (t) = 
%		%	\begin{cases}
%		%		P_\mathrm{fd}(t) \cdot \eta_\mathrm{fgt}^{-sign(P_\mathrm{fd}(t))} & \text{~~if FGT,} \\
%		%		P_\mathrm{fd}(t) \cdot \eta_\mathrm{cvt}^{-sign(P_\mathrm{fd}(t))} & \text{~~if CVT,}
%		%	\end{cases}
%		P_\mathrm{m} \geq \text{max} \Big( \frac{1}{\eta_\mathrm{gb} \cdot \eta_\mathrm{fd}} \cdot P_\mathrm{fd}, 
%				\eta_\mathrm{gb} \cdot \eta_\mathrm{fd} \cdot r_\mathrm{b} \cdot P_\mathrm{fd} \Big)
%	\end{equation}
%\end{small}
%\endgroup
The rotational speed of the motor shaft for a given gear ratio $\gamma$ is calculated using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:W_to_MOt_Speed}
%		\omega_{\mathrm{mot}}(t) = \gamma(t) \cdot \gamma_{\mathrm{fd}} \cdot \frac{v(t)}{r_{\mathrm{w}}}, 
		\omega_{\mathrm{m}} = \gamma \cdot \gamma_{\mathrm{fd}} \cdot \dfrac{v(t)}{r_{\mathrm{w}}}, 
	\end{equation}
\end{small}%
\endgroup
where $r_{\mathrm{w}}$ is the radius of the wheel and $\gamma_{\mathrm{fd}}$ is the final drive gear ratio, and $\gamma$ is the transmission gear ratio. The transmission ratio is one of the optimization variables and depending on the type of transmission, it is constrained as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}%
		\label{eq:gamma_Limits}
		\gamma(t) 
%		\gamma 
		\begin{cases}
			= \gamma_\mathrm{fgt} &\forall~t~~\text{ if  FGT},   \\
			\in [\gamma_{\mathrm{min}}, \gamma_{\mathrm{max}}]  & \forall~t~~\text{ if  CVT}.  
		\end{cases}
	\end{equation}
\end{small}%
\endgroup
Finally, the total mass of the vehicle is
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}%
		\label{eq:Mass}
		m_{\mathrm{v}} = m_{\mathrm{0}} + m_{\mathrm{m}} +  
		\begin{cases}
			m_{\mathrm{fgt}} &\text{ if  FGT},   \\
			m_{\mathrm{cvt}} &\text{ if  CVT},  
		\end{cases}
	\end{equation}
\end{small}%
\endgroup
where $m_{\mathrm{0}}$ is the base mass of the vehicle, $m_{\mathrm{m}}$ is the mass of the motor, $m_{\mathrm{fgt}}$ is the mass of the FGT and $m_{\mathrm{cvt}}$ is the mass of the CVT. We assume that the base mass includes the mass of the frame, the battery mass and the equivalent mass due to the moment of inertia of rotating parts.



\subsection{Electric Motor and Inverter}\label{sec:methodology_motor}
\ifextendedversion
In this section, we derive a temperature-independent model and an accurate temperature-dependent model of the EM losses inspired from our previous work~\cite{LocatelloKondaEtAl2020,HurkSalazar2021}. The former model will be leveraged to calculate an initial guess for a detailed temperature-dependent model. 
\else
In this section, we derive an accurate temperature-dependent model of the EM losses inspired from our previous work~\cite{LocatelloKondaEtAl2020,HurkSalazar2021}. 
\fi
One of the most common types of motors for a light passenger vehicle is an Interior Permanent Magnet (IPM) motor~\cite{MK_HwangHan2018Design}. We model the IPM motor based on the templates provided in the high-fidelity simulation software Motor-CAD. We use the data generated by the software to identify and validate the motor loss models and motor thermal models. Subsequently, the power at the motor terminals $P_\mathrm{inv}$ is given by
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}%
		\label{eq:MOT_Power_Balance}
		P_{\mathrm{inv}} = P_{\mathrm{m}} + P_{\mathrm{loss}},
		\end{equation}
\end{small}%
\endgroup
where $P_{\mathrm{loss}}$ represents the total losses in the motor and can be defined as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}%
		\label{eq:MOT_Ploss_total}
%		P_{\mathrm{loss}} = P_{\mathrm{sft}} + P_{\mathrm{rtr}} + P_{\mathrm{mgt}} + P_{\mathrm{str}} + P_{\mathrm{wdg}}
%		P_{\mathrm{loss}} = \sum_\mathrm{i} P_{\mathrm{i}}~~~~~\forall~~~\{\text{i = sft, rtr, mgt, str, wdg}\}
		P_{\mathrm{loss}} = \sum_i P_i,~~~~~\forall~~~\{i = \text{sft, rtr, mgt, str, wdg}\},
	\end{equation}
\end{small}%
\endgroup
where $P_{i}$ represents the losses corresponding to the components of the motor, namely the shaft (sft), the rotor (rtr), the permanent magnets (mgt), the stator (str) and the windings (wdg). \mkmargin{The losses are individually identified for each EM component in order to build an LPTN and explicitly capture the thermal dynamics of the EM, which will be discussed in Section~\ref{sec:methodology_thermal}}{required?}. The shaft losses, $P_\mathrm{sft}$, are independent of motor power and temperature. Therefore, we compute them using the linear relation
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Shaft_Losses}
		\begin{aligned}
			%		x_\mathrm{sft}(t) &= \begin{bmatrix}
			%			1 & \omega_{\mathrm{m}}(t)
			%		\end{bmatrix}^\top \\
			%		P_\mathrm{sft}(t) &= a_\mathrm{sft} \cdot x_\mathrm{sft}(t) 
			P_\mathrm{sft} &= a_\mathrm{sft,0} + a_\mathrm{sft,1} \cdot \omega_{\mathrm{m}},
		\end{aligned}
	\end{equation}
\end{small}%
\endgroup
%\begin{equation*}
%	\begin{aligned}
%		P_\mathrm{req} & < 0, \\
%		& P_\mathrm{i}  = x_\mathrm{i}(t)^\top~Q_\mathrm{i}~x_\mathrm{i}(t) \\
%		& \mathrm{i}    = \mathrm{rtr, mgt, str, wdg} \\ 			
%		& x_\mathrm{i}(t) = \begin{bmatrix}
%			1 & \omega_{\mathrm{m}}(t) & P_{\mathrm{m}}(t) & \omega_{\mathrm{m}}(t)^2 & P_{\mathrm{m}}(t)^2 & \omega_{\mathrm{m}}(t) \cdot P_{\mathrm{m}}(t) \end{bmatrix} \\
%	\end{aligned}
%\end{equation*}
where $a_\mathrm{sft}$ is subject to identification. 
\ifextendedversion
We estimate the temperature-independent losses of the other components by using convex quadratic functions of the form $P_i  = x^\top~Q_i~x$, for $i \in \{\text{rtr, mgt, str, wdg}\}$, where $Q_i$ is a positive semi-definite matrix and $x = \begin{bmatrix} 1 & \omega_{\mathrm{m}} & P_{\mathrm{m}} & \omega_{\mathrm{m}}^2 & P_{\mathrm{m}}^2 & \omega_{\mathrm{m}} \cdot P_{\mathrm{m}} \end{bmatrix} ^\top$. The maps are identified using the data generated by Motor-CAD at an EM temperature of $65\unit{^{\circ}C}$. In order to ensure convexity, we relax the losses to
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks
%\begin{small} 
%	\label{eq:EM_loss_simple1}
%	\begin{equation}
%%		\begin{aligned}
%%			P_\mathrm{req} & < 0, \\
%%			P_\mathrm{i}  &= x_\mathrm{i}^\top~Q_\mathrm{i}~x_\mathrm{i} \\
%%			& \mathrm{i}    = \mathrm{rtr, mgt, str, wdg} \\ 			
%%			& x_\mathrm{i} = \begin{bmatrix}
%%				1 & \omega_{\mathrm{m}} & P_{\mathrm{m}} & \omega_{\mathrm{m}}^2 & P_{\mathrm{m}}^2 & \omega_{\mathrm{m}} \cdot P_{\mathrm{m}} \end{bmatrix} \\
%%			&~~Q \geq 0
%%		\end{aligned}
%		P_\mathrm{i} \geq x_\mathrm{i}^\top~Q_\mathrm{i}~x_\mathrm{i}
%	\end{equation}
%\end{small}
%\endgroup
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small} 
	\begin{equation}
		\label{eq:EM_loss_simple1}
%		P_\mathrm{i} \geq x_\mathrm{i}^\top~Q_\mathrm{i}~x_\mathrm{i}
		P_i \geq x^\top Q_i x.
	\end{equation}
\end{small}%
\endgroup
This constraint will hold with equality in a case where the solver converges to an optimal solution. Subsequently, we present the state-of-the-art motor loss models for which we categorize the driving cycle into two scenarios: traction and braking.
\else
Now, we present the loss models for the other EM components for which we categorize the driving cycle into two scenarios: traction and braking.
\fi
During traction, the motor must supply the full power required to propel the vehicle. In contrast, when braking, we can split the power between friction brakes and regenerative braking to keep the EM's temperatures within their limits. The main advantage of this model is that, for a given drive cycle, the motor power is known in the traction phases, which enables us to accurately model the EM losses by using motor-power-level-specific fitting coefficients, thereby improving the accuracy of the models compared to~\cite{LocatelloKondaEtAl2020}. We compute the minimum tractive power required to propel the vehicle, $\overline{P}_\mathrm{m}$, using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Pm_bar}
		\overline{P}_\mathrm{m} = \text{max} \Big( \dfrac{1}{\eta_\mathrm{gb} \cdot \eta_\mathrm{fd}} \cdot P_\mathrm{req}, 
		\eta_\mathrm{gb} \cdot \eta_\mathrm{fd} \cdot r_\mathrm{b} \cdot P_\mathrm{req}, {P}_\mathrm{m,min} \Big).
	\end{equation}
\end{small}%
\endgroup
%Whilst during braking, the power flows from the wheels to the EM. In this case, we can control the amount of power recuperated by the EM to maintain the temperature of EM within its limits. This can be done by diverting partial or full power from the wheels to mechanical brakes. The advantage of these models is that the tractive motor power can be precomputed and the loss model coefficients can be identified for each power level thereby drastically improving the accuracy of models compared to~\cite{LocatelloKondaEtAl2020}.
%Since, the motor power is known in advance, we can improve the accuracy of power loss models by identifying the coefficients at each power level.
%We must note that the coefficients to compute these losses are identified for every motor power in the drive cycle. The minimum motor power required to propel the vehicle, $\overline{P}_\mathrm{m}$, is given by
To avoid repetition, we present the relaxed versions of the motor power loss equations. First, the rotor and stator losses are computed using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		\label{eq:Rtr_Loss_Complex}
%		\begin{aligned}
			P_\mathrm{rtr} \geq \\
			\begin{cases}
				a_\mathrm{rtr,0}(\overline{P}_\mathrm{m}) + 
				a_\mathrm{rtr,1}(\overline{P}_\mathrm{m}) \cdot \omega_{\mathrm{m}} + 
				a_\mathrm{rtr,2}(\overline{P}_\mathrm{m}) \cdot \omega_{\mathrm{m}}^2,\\
				\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \text{if} ~ \overline{P}_\mathrm{m} \geq 0,\\
				y^\top Q_\mathrm{rtr} y, \qquad \qquad \qquad \qquad \qquad \qquad ~~~~~ \text{if} ~ \overline{P}_\mathrm{m} < 0,\\
			\end{cases}\\
%		\end{aligned}
	\end{equation}
\end{small}%
\endgroup
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks
%\begin{small}
%	\begin{equation}
%		\label{eq:Rtr_Loss_Complex}
%		P_\mathrm{rtr} \geq
%		\begin{cases}
%			a_\mathrm{rtr,0} + 
%			a_\mathrm{rtr,1} \cdot \omega_{\mathrm{m}} + 
%			a_\mathrm{rtr,2} \cdot \omega_{\mathrm{m}}^2, &\quad \overline{P}_\mathrm{m} \geq 0\\
%			x^\top \cdot Q_\mathrm{rtr} \cdot x,          &\quad \overline{P}_\mathrm{m} < 0
%		\end{cases}
%	\end{equation}
%\end{small}
%\endgroup%
\par\nobreak\vspace{-15pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		\label{eq:Str_Loss_Complex}
%		\begin{aligned}
			P_\mathrm{str} \geq \\
			\begin{cases} 
				a_\mathrm{str,0}(\overline{P}_\mathrm{m}) + 
				a_\mathrm{str,1}(\overline{P}_\mathrm{m}) \cdot \omega_{\mathrm{m}} + 
				a_\mathrm{str,2}(\overline{P}_\mathrm{m}) \cdot \omega_{\mathrm{m}}^2,\\
				\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \text{if} ~ \overline{P}_\mathrm{m} \geq 0,\\
				y^\top Q_\mathrm{str} y, \qquad \qquad \qquad \qquad \qquad \qquad ~~~~~ \text{if} ~ \overline{P}_\mathrm{m} < 0,\\
			\end{cases}\\
%		\end{aligned}
	\end{equation}
\end{small}%
\endgroup
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks
%\begin{small}
%	\begin{equation}
%		\label{eq:Str_Loss_Complex}
%		\begin{aligned}
%			& P_\mathrm{str} \geq
%			& \begin{cases}
%				a_\mathrm{str,0} + 
%				a_\mathrm{str,1} \cdot \omega_{\mathrm{m}} + 
%				a_\mathrm{str,2} \cdot \omega_{\mathrm{m}}^2, &\quad \overline{P}_\mathrm{m} \geq 0\\
%				x^\top \cdot Q_\mathrm{str} \cdot x,          &\quad \overline{P}_\mathrm{m} < 0, \\
%			  \end{cases}\\
%		\end{aligned}
%	\end{equation}
%\end{small}
%\endgroup
where $a_\mathrm{rtr}$ and $a_\mathrm{str}$ are subject to identification and $y = \begin{bmatrix} 1 & \omega_{\mathrm{m}} & P_{\mathrm{m}} & \omega_{\mathrm{m}}^2 & P_{\mathrm{m}}^2 & \omega_{\mathrm{m}} \cdot P_{\mathrm{m}} \end{bmatrix} ^\top$. To retain convexity in the positive speed domain, we ensure that $a_\mathrm{rtr,2}~\geq~0$ and $a_\mathrm{str,2}~\geq~0$. Second, the magnet loss models are temperature-dependent and computed using convex quadratic relations of the form
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		\label{eq:Mgt_Loss_Complex}
		P_\mathrm{mgt} \geq 
		\begin{cases}
			z_\mathrm{mgt}^\top~R_\mathrm{mgt}(\overline{P}_\mathrm{m})~z_\mathrm{mgt}, &\quad \overline{P}_\mathrm{m} \geq 0,\\
			x^\top Q_\mathrm{mgt} x, &\quad \overline{P}_\mathrm{m} < 0,
		\end{cases}
	\end{equation}
\end{small}%
\endgroup
where $R_\mathrm{mgt}$ is a positive semi-definite matrix, subject to identification and $z_\mathrm{mgt} = \begin{bmatrix} 1 & \omega_{\mathrm{m}} & \vartheta_{\mathrm{mgt}} \end{bmatrix} ^\top$. Third, the temperature-dependent winding losses are given by
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		\label{eq:Wdg_Loss_Complex}
%		\begin{aligned}
			P_\mathrm{wdg} \geq \\ 
			\begin{cases}
				z_\mathrm{wdg}^\top~R_\mathrm{wdg}(\overline{P}_\mathrm{m})~z_\mathrm{wdg} + 
				\dfrac{a_\mathrm{wdg,1}(\overline{P}_\mathrm{m})}{\omega_\mathrm{m}} + 
				\dfrac{a_\mathrm{wdg,2}(\overline{P}_\mathrm{m})}{\omega_\mathrm{m}^2}, \\
				\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \text{if} ~ \overline{P}_\mathrm{m} \geq 0,\\
				x^\top Q_\mathrm{wdg} x, \qquad \qquad \qquad \qquad \qquad \qquad ~~~~ \text{if} ~ \overline{P}_\mathrm{m} < 0,\\
			\end{cases}	\\	
%		\end{aligned}		
	\end{equation}
\end{small}%
\endgroup
where $a_\mathrm{wdg}$ and $R_\mathrm{wdg}$ are subject to identification and $z_\mathrm{wdg} = \begin{bmatrix} 1 & \omega_{\mathrm{m}} & \vartheta_{\mathrm{wdg}} & \omega_{\mathrm{m}}^2 & \vartheta_{\mathrm{wdg}}^2 & \omega_{\mathrm{m}} \cdot \vartheta_{\mathrm{wdg}} \end{bmatrix} ^\top$. In addition, we ensure that   $a_\mathrm{wdg,1} \geq 0$, $a_\mathrm{wdg,2} \geq 0$, and $R_\mathrm{wdg}$ is a positive semi-definite matrix to preserve convexity in the positive speed domain. To prevent the winding losses from reaching infinity when the vehicle is starting, we set $a_\mathrm{wdg,1} = 0$ and $a_\mathrm{wdg,2} = 0$ at very low speeds. 
\ifextendedversion
The advanced rotor, stator, magnet and winding losses for three different motor power levels are shown in Appendix~\ref{app:Motor_Loss}. 
\else
Moreover, we constrain the power losses with %\mkmargin{The motor loss model can be finally summarized as}{write more clearly, also introduce it above.}
\fi
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:MOT_Loss_geq0}
		P_{i} \geq 0, ~~~~~\forall~~~\{i = \text{sft, rtr, mgt, str, wdg}\}.
	\end{equation}
\end{small}%
\endgroup
%\par\nobreak\vspace{-5pt}
%\begingroup
%\allowdisplaybreaks 
%\begin{small}
%	\begin{equation}
%		\label{eq:MOT_Loss_Final}
%		P_i = 
%		\begin{cases}
%			Eq.~\ref{eq:Shaft_Losses},~\ref{eq:Rtr_Loss_Complex},~\ref{eq:Str_Loss_Complex},~\ref{eq:Mgt_Loss_Complex},~\ref{eq:Wdg_Loss_Complex}&~~~\text{if}~~P_\mathrm{m}\geq 0 \\
%			Eq.~\ref{eq:Shaft_Losses},~\ref{eq:EM_loss_simple1}&~~~\text{if}~~P_\mathrm{m}<0		
%		\end{cases}
%	\end{equation}
%\end{small}
%\endgroup
\begin{figure}[t!]	
	\centering
	\includegraphics[trim=1.2cm 0.4cm 1.65cm 0.25cm,clip=true, width=\columnwidth]{img/Efficiency_Data_Model.pdf}
	\caption{Efficiency map of the interior permanent magnet (IPM) machine (left) and its convex model (right) at a temperature of \unit[65]{$^{\circ}$C}. }
	\label{fig:Efficiency_Data_Model}
\end{figure}%
\ifextendedversion
\begin{figure}[t!]	
	\centering
	\includegraphics[trim=2cm 1.5cm 1.5cm 1.5cm,clip=true, width=\columnwidth]{img/Ploss_Data_Model.pdf}
	\caption{ The power loss models of various motor components. Speed-dependent shaft losses with $\mathrm{NRMSE}_{\mathrm{sft}} = 0\%$ (top left); speed-, power-dependent  rotor and stator losses with $\mathrm{NRMSE}_{\mathrm{rtr}} = 1.5\%$ (top right) and $\mathrm{NRMSE}_{\mathrm{str}} = 3.4\%$ (center right); speed-, power-, temperature-dependent magnet and winding losses with $\mathrm{NRMSE}_{\mathrm{mgt}} = 1.4\%$ (center left) and $\mathrm{NRMSE}_{\mathrm{wdg}} = 5.4\%$ (bottom). }
	\label{fig:Ploss_Data_Model}
\end{figure}%
\fi
% RMSE_sf = 8.0923e-10%, RMSE_rtr = 1.4599%, RMSE_str = 3.4318%, RMSE_mgt = 1.4077%, RMSE_wdg = 5.3957%
The relaxed constraints will hold with equality in the case where an optimal solution is attained. 
\ifextendedversion
Fig.~\ref{fig:Efficiency_Data_Model} compares the efficiency map obtained from Motor-CAD with the efficiency map from convex models, whilst Fig.~\ref{fig:Ploss_Data_Model} shows the resulting power loss models. We can observe that the models are accurate, especially in the positive domain where most of the operation occurs and the motor-power-level-specific model is more precise. The normalized root mean squared error of the winding losses is higher than other components because of the slightly inaccurate fit at low speeds and negative torques which can be seen from bottom subfigure of Fig.~\ref{fig:Ploss_Data_Model}. Furthermore, the normalized loss prediction error with respect to the data from Motor-CAD is in the order of 5\%, resulting in a total error in input power prediction of less than 1\%.
\else
Fig.~\ref{fig:Efficiency_Data_Model} compares the efficiency map obtained from Motor-CAD with the efficiency map from convex models. We can observe that the models are accurate, especially in the positive domain where most of the operation occurs.
\fi
The torque limits of the EM are 
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:MOT_Torque_Limit}
		P_{\mathrm{m}} \in \left[T_\mathrm{m,min}, T_\mathrm{m,max}\right] \cdot \omega_{\mathrm{m}},
	\end{equation}
\end{small}%
\endgroup
\ifextendedversion
where $T_\mathrm{m,max}$ and $T_\mathrm{m,min}$ are the maximum and minimum torques subject to identification as shown in Appendix~\ref{app:Motor_Limits}.
\else
where $T_\mathrm{m,max}$ and $T_\mathrm{m,min}$ are the maximum and minimum torques subject to identification.
\fi
In addition, we bound the EM power as 
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:MOT_Power_Limit}
		\begin{aligned}
			P_{\mathrm{m}} &\in \left[P_{\mathrm{m,min}}, P_{\mathrm{m,max}}\right],\\
%			&\left[d_\mathrm{1,min} \cdot \omega_{\mathrm{m}} + d_\mathrm{0,min}, d_\mathrm{1,max} \cdot \omega_{\mathrm{m}} + d_\mathrm{0,max}\right],
		\end{aligned}		
	\end{equation}
\end{small}%
\endgroup
\ifextendedversion
where $P_{\mathrm{m,min}}$ and $P_{\mathrm{m,max}}$ are the minimum and maximum motor powers, respectively. We compute them using the relations $P_{\mathrm{m,min}}~=~d_\mathrm{1,min}~\cdot~\omega_{\mathrm{m}}~+~d_\mathrm{0,min}$, $P_{\mathrm{m,max}}~=~d_\mathrm{1,max}~\cdot~\omega_{\mathrm{m}}~+~d_\mathrm{0,max}$ where $d_\mathrm{0,min}$, $d_\mathrm{1,min}$, $d_\mathrm{1,max}$ and $d_\mathrm{1,max}$ are the coefficients subject to identification as shown in Appendix~\ref{app:Motor_Limits}.
\else
where $P_{\mathrm{m,min}}$ and $P_{\mathrm{m,max}}$ are the minimum and maximum motor powers, respectively. We compute them using the relations $P_{\mathrm{m,min}}~=~d_\mathrm{1,min}~\cdot~\omega_{\mathrm{m}}~+~d_\mathrm{0,min}$, $P_{\mathrm{m,max}}~=~d_\mathrm{1,max}~\cdot~\omega_{\mathrm{m}}~+~d_\mathrm{0,max}$ where $d_\mathrm{0,min}$, $d_\mathrm{1,min}$, $d_\mathrm{1,max}$ and $d_\mathrm{1,max}$ are the coefficients subject to identification.
\fi
The non-negative rotational speed of the motor is bounded by the maximum EM speed, $\omega_{\mathrm{m,max}}$, as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:MOT_Speed_Limit}
		\omega_{\mathrm{m}} \in \left[0, \omega_{\mathrm{m,max}}\right].
	\end{equation}
\end{small}%
\endgroup
Finally, we approximate the inverter losses using the quadratic function
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:INV_BAT_Losses}
		P_{\mathrm{dc}} = 	\alpha_\mathrm{inv} \cdot P_{\mathrm{inv}}^2 + P_{\mathrm{inv}},
	\end{equation}
\end{small}%
\endgroup
where $\alpha_\mathrm{inv}$ is the inverter coefficient subject to identification,
\ifextendedversion
$P_{\mathrm{dc}}$ is the output power at the battery terminals (see Appendix~\ref{app:Inveter_Loss}).
\else
$P_{\mathrm{dc}}$ is the output power at the battery terminals.
\fi
To preserve convexity, we relax Eq.~\ref{eq:INV_BAT_Losses} to $ P_{\mathrm{dc}} \geq 	\alpha_\mathrm{inv} \cdot P_{\mathrm{inv}}^2 + P_{\mathrm{inv}} $.


\subsection{Motor Thermal Model and Fan Model}\label{sec:methodology_thermal}
\begin{figure}[t!]
	\centering
	\includegraphics[trim=0.5cm 0.25cm 0.25cm 0cm,clip=true, width=\columnwidth]{img/Motor3d_ThermalNetwork.pdf}
%	\includegraphics[trim=0.5cm 0.25cm 0.25cm 18cm,clip=true, width=\columnwidth]{img/Motor3d_ThermalNetwork.pdf}
	%\caption{A 3-dimensional section view of the IPM motor from Motor-CAD (top) and its Lumped Parameter Thermal Network (bottom).}
	\caption{The Lumped Parameter Thermal Network of the IPM motor.}
	\label{fig:ThermalNetwork}
\end{figure}%
\begin{table}[t!]
	\caption{Thermal limits of the nodes of the thermal network}
	\centering
	\begin{tabular}{l c l c}
		\toprule
		Component  & $\vartheta_{i,\mathrm{max}}$ [\unit{$^ \circ$C}] & Component  & $\vartheta_{i,\mathrm{max}}$ [\unit{$^ \circ$C}]\\
		\hline
		Shaft          & 140 & Permanent Magnets        & 120 \\
		Rotor          & 140 & Stator                   & 140 \\
		Windings       & 160 & End-windings             & 160 \\
		\bottomrule
	\end{tabular}
	\label{tab:ThLim}
\end{table}%
In this section, we derive an LPTN model, based on~\cite{LocatelloKondaEtAl2020,MK_WeiHofman2021CoDesign,MK_WangJagarwal2014Optimization}. In addition to the EM components presented in Section~\ref{sec:methodology_motor}, we include the overhanging copper windings, further referred to as end-windings (edwg), in our thermal model because the end-windings reach higher temperatures and are the limiting factors in high-performance operations~\cite{MadonnaWalkerEtAl2018}. Therefore, we build the LPTN with a total of 6 nodes: the shaft (sft), the rotor (rtr), the permanent magnets (mgt), the stator (str), the windings (wdg) and the end-windings (edwg). The LPTN is based on the following assumptions: First, the heat flow in the radial direction is independent of the heat flow in the axial direction. Second, the heat flow in the circumferential direction is absent. Third, each component's thermal properties, including its temperature, can be represented by a single node, i.e., the temperature distribution in a component is uniform. Fig.~\ref{fig:ThermalNetwork} shows the cross-section of the IPM machine at the top and its LPTN at the bottom. The energy balance equations for the LPTN are given by 
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
 \begin{small}
	\begin{equation}
%	 	\label(eq:Thermal_Dynamics)
%		\left
		\begin{aligned}
			P_{\mathrm{sft}} &= c _{\mathrm{sft}}  \dot{\vartheta}_{\mathrm{sft}} + 
								  k_{\mathrm{sft,rtr}} (\vartheta_{\mathrm{sft}} - \vartheta_{\mathrm{rtr}}) \\
			P_{\mathrm{rtr}} &= c _{\mathrm{rtr}}  \dot{\vartheta}_{\mathrm{rtr}} + 
								  k_{\mathrm{sft,rtr}} (\vartheta_{\mathrm{rtr}} - \vartheta_{\mathrm{sft}}) + 
								  k_{\mathrm{rtr,mgt}} (\vartheta_{\mathrm{rtr}} - \vartheta_{\mathrm{mgt}})  \\  
							   &  \quad + k_{\mathrm{rtr,str}} (\vartheta_{\mathrm{rtr}} - \vartheta_{\mathrm{str}}) + 
								  k_{\mathrm{rtr,wdg}} (\vartheta_{\mathrm{rtr}} - \vartheta_{\mathrm{wdg}})\\
			P_{\mathrm{mgt}} &= c_{\mathrm{mgt}}  \dot{\vartheta}_{\mathrm{mgt}} + 
							      k_{\mathrm{rtr,mgt}} (\vartheta_{\mathrm{mgt}} - \vartheta_{\mathrm{rtr}}) \\
			P_{\mathrm{str}} &= c_{\mathrm{str}}  \dot{\vartheta}_{\mathrm{str}} + 
								  k_{\mathrm{rtr,str}} (\vartheta_{\mathrm{str}} - \vartheta_{\mathrm{rtr}}) + 
								  k_{\mathrm{str,wdg}} (\vartheta_{\mathrm{str}} - \vartheta_{\mathrm{wdg}}) \\ 
							   &  \quad + k_{\mathrm{str,col}} (\vartheta_{\mathrm{str}} - \vartheta_{\mathrm{col}})\\
			P_{\mathrm{wdg}} &= c_{\mathrm{wdg}}  \dot{\vartheta}_{\mathrm{wdg}} + 
								  k_{\mathrm{str,wdg}} (\vartheta_{\mathrm{wdg}} - \vartheta_{\mathrm{str}})\\
							   &  \quad + k_{\mathrm{rtr,wdg}} (\vartheta_{\mathrm{wdg}} - \vartheta_{\mathrm{rtr}}) + 
								  k_{\mathrm{wdg,ewdg}} (\vartheta_{\mathrm{wdg}} - \vartheta_{\mathrm{ewdg}})\\
			P_{\mathrm{wdg}} &= c_{\mathrm{ewdg}}  \dot{\vartheta}_{\mathrm{ewdg}} + 
								  k_{\mathrm{wdg,ewdg}} (\vartheta_{\mathrm{ewdg}} - \vartheta_{\mathrm{wdg}}),
		\end{aligned}	%\right.
	\end{equation}
\end{small}%
\endgroup
where $\vartheta_i$ and $\dot{\vartheta}_i$ represent the temperature of a node and the rate of change of temperature, respectively, for the nodes, $i \in \{ \text{sft, rtr, mgt, str, wdg, ewdg} \} $. Parameter $k_{i,j}$ represents the overall heat transfer coefficient between node $i$ and node $j$, and $c_i$ represents the heat capacity of the node.  Parameters $k_{i,j}$ and $c_i$ are subject to identification. We use nonlinear gradient-based methods to identify the thermal coefficients. In addition, we use the losses estimated by our power loss models instead of the losses from the high-fidelity software to avoid propagating the error of the power loss model to the LPTN.
\ifextendedversion
The LPTN fitting is shown in Appendix~\ref{app:Thermal_Fitting} and the collective fitting error is 0.62\%. 
\fi
In order to prevent motor failure due to thermal limitations, we constrain the temperature of each node using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Thermal_Limits}
		\vartheta_i \leq \vartheta_{i,\mathrm{max}},
	\end{equation}
\end{small}%
\endgroup
where $\vartheta_{i,\mathrm{max}}$ is the temperature limit of node $i$. Table~\ref{tab:ThLim} summarizes the maximum temperatures of all the nodes. We simulate the vehicle by initializing the temperature of each node at the coolant temperature, $\vartheta_{\mathrm{col}}$, as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:T_start}
		\vartheta_{i}(0) = \vartheta_{\mathrm{col}}.
	\end{equation}
\end{small}%
\endgroup
Finally, the air flow rate, $\dot{m}_{\mathrm{air}}$, required by the fan to remove heat is given by
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:FAN_air}
%		\dot{m}_{\mathrm{air}}(t) = \frac{k_{\mathrm{st,col}} (\vartheta_{\mathrm{str}} - \vartheta_{\mathrm{col}} + P_\mathrm{loss,inv}(t) + P_\mathrm{loss,tra}(t) }{\epsilon \cdot C_\mathrm{p,air} \cdot \Delta T} 
%		\dot{m}_{\mathrm{air}} = \frac{k_{\mathrm{str,col}} (\vartheta_{\mathrm{str}} - \vartheta_{\mathrm{col}}) + 		P_\mathrm{loss,inv} + P_\mathrm{loss,tra} }{\epsilon \cdot C_\mathrm{p,air} \cdot \Delta T},
		\dot{m}_{\mathrm{air}} = \frac{ P_\mathrm{mot,rej} + 	P_\mathrm{loss,inv} + P_\mathrm{loss,tra} }{\eta_\mathrm{he} \cdot C_\mathrm{p,air} \cdot \Delta \vartheta_{\mathrm{a}}},
	\end{equation}
\end{small}%
\endgroup
where the transmission losses are $P_\mathrm{loss,tra}~=~P_\mathrm{m}~-~P_\mathrm{fd}$, the inverter losses are given as $P_\mathrm{loss,inv}~=~P_\mathrm{dc}~-~P_\mathrm{inv}$ and the heat rejected by the EM is $P_\mathrm{mot,rej}~=~k_{\mathrm{str,col}}~(\vartheta_{\mathrm{str}}~-~\vartheta_{\mathrm{col}})$. In addition, $\eta_\mathrm{he}$ is the heat exchanger efficiency, $C_\mathrm{p,air}$ is the specific heat capacity of air and $\Delta \vartheta_{\mathrm{a}}$ is the constant temperature gain of the air across the radiator~\cite{MK_WangJagarwal2014Optimization}. We compute the power required by the fan, $P_\mathrm{fan}$, using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:FAN_Power}
		P_{\mathrm{fan}} = \alpha_{\mathrm{f}} \cdot \dot{m}_{\mathrm{air}}^2,
	\end{equation}
\end{small}%
\endgroup
\ifextendedversion
where $\alpha_{\mathrm{f}}$ is again subject to identification as shown in Appendix~\ref{app:Fan_fitting}. %\mkmargin{the fan model was kept simple without a constant because we want to emulate the power when fan is switched off. It was a concious descision. And this approach was taken because the fan losses are propotional to sqaure of fan speed.}{}
\else
where $\alpha_{\mathrm{f}}$ is again subject to identification and to preserve convexity the equation is relaxed to $P_{\mathrm{fan}} \geq \alpha_{\mathrm{f}} \cdot \dot{m}_{\mathrm{air}}^2$. The maximum air flow rate is constrained as  $\dot{m}_{\mathrm{air}} \leq \dot{m}_{\mathrm{air,max}}$.
\fi

\subsection{Battery}\label{sec:methodology_battery}
In this section, we derive two battery models: an energy independent model and a more detailed energy-dependent model. The first model will provide an initial guess, whilst the latter will capture the battery dynamics accurately. Even though modeling and identification of battery dynamics is not part of this thesis, they are included for completeness in line with~\cite{VerbruggenSalazarEtAl2019}. First, the electric power at the battery terminals, $P_{\mathrm{bat}}$, is computed as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:INV_BAT_AUX_Equillibrium}	
%		P_{\mathrm{bat}}(t) = P_{\mathrm{dc}}(t) + P_{\mathrm{aux}}(t)
		P_{\mathrm{bat}} = P_{\mathrm{dc}} + P_{\mathrm{aux}} + P_{\mathrm{fan}},
	\end{equation}
\end{small}%
\endgroup
where $P_{\mathrm{aux}}$ is the auxiliary power. Then, we approximate the battery losses with the quadratic function
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:BAT_INT_Losses}
%		P_{\mathrm{int}}(t) = \alpha_{\mathrm{b}} \cdot P_{\mathrm{int}}(t) + P_{\mathrm{int}}(t)
		P_{\mathrm{int}} = \alpha_{\mathrm{b}} \cdot P_{\mathrm{bat}}^2 + P_{\mathrm{bat}},
	\end{equation}
\end{small}%
\endgroup
where $\alpha_{\mathrm{b}}$ is subject to identification (see Appendix~\ref{app:Battery_Fitting}), and $P_{\mathrm{int}}$ is the internal power of the battery which changes the battery state of energy (SoE). Subsequently, in line with~\cite{VerbruggenSalazarEtAl2019}, we model the energy-dependent battery dynamics using
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:BAT_INT_Losses_Complex}
%		(P_{\mathrm{int}}(t) - P_{\mathrm{bat}}(t)) \cdot P_{\mathrm{oc}}(t) = P_{\mathrm{int}}(t)^2
		(P_{\mathrm{int}} - P_{\mathrm{bat}}) \cdot P_{\mathrm{oc}} = P_{\mathrm{int}}^2,
	\end{equation}
\end{small}%
\endgroup
where $P_{\mathrm{oc}}$ is the open circuit power dependent on the internal resistance of the battery and its open circuit voltage. To preserve convexity, we relax Eq.~\ref{eq:BAT_INT_Losses_Complex} as $(P_{\mathrm{int}}~-~P_{\mathrm{bat}})~\cdot~P_{\mathrm{oc}}~\geq~P_{\mathrm{int}}^2$ which, again, will hold with equality when the solver converges to an optimal solution. Furthermore, $P_{\mathrm{oc}}$ is a function of the (SoE) of the battery and defined as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Poc_Linear_Eq}
%		P_{\mathrm{oc}}(t) = b_1 \cdot E_{\mathrm{b}}(t) + b_2 \cdot E_{\mathrm{b,max}}
		P_{\mathrm{oc}} = b_\mathrm{1} \cdot E_{\mathrm{b}} + b_\mathrm{2} \cdot E_{\mathrm{b,max}},
	\end{equation}
\end{small}%
\endgroup
where $b_\mathrm{1}$ and $b_\mathrm{2}$ are subject to identification. $ P_{\mathrm{int}} $ is bounded between
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Pint_Limits}
%		P_{\mathrm{int}}(t) \in \left[ P_{\mathrm{int,min}}, P_{\mathrm{int,max}}\right]
		P_{\mathrm{int}} \in \left[ -P_{\mathrm{int,max}}, P_{\mathrm{int,max}}\right],
	\end{equation}
\end{small}%
\endgroup
where $P_{\mathrm{int,max}}$ is the maximum internal power of the battery. It is dependent on SoE as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Pint_Fitting}
%		P_{\mathrm{int}}(t) = c_1 \cdot E_{\mathrm{b}}(t) + c_2 \cdot E_{\mathrm{b,max}}
		P_{\mathrm{in,maxt}} = c_\mathrm{1} \cdot E_{\mathrm{b}}(t) + c_\mathrm{2} \cdot E_{\mathrm{b,max}},
	\end{equation}
\end{small}%
\endgroup
where $c_\mathrm{1}$ and $c_\mathrm{2}$ are again subject to identification. Additionally, we bound the battery SoE between the minimum and maximum state of charge (SoC) levels, $\zeta_{\mathrm{b,min}}$ and $\zeta_{\mathrm{b,max}}$, respectively, as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:BAT_SOC_Limit}
%		E_\mathrm{b}(t) \in \left[ \zeta_{\mathrm{b,min}}, \zeta_{\mathrm{b,max}}\right]
		E_\mathrm{b} \in \left[ \zeta_{\mathrm{b,min}}, \zeta_{\mathrm{b,max}}\right] \cdot E_{\mathrm{b,max}}.
	\end{equation}
\end{small}%
\endgroup
We consider that the vehicle starts with a full battery at the start of the cycle. Mathematically, it can be represented as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Battery_Initial}
		E_\mathrm{b}(0) = E_\mathrm{b,max} \cdot \zeta_{\mathrm{b,max}}.
	\end{equation}
\end{small}%
\endgroup
Finally, the battery SoE changes with $P_\mathrm{int}$ as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Battery_Dynamics}
%		\frac{\mathrm{d}}{\mathrm{d}t}E_\mathrm{b}(t) = -P_\mathrm{int}(t)
		\frac{\mathrm{d}}{\mathrm{d}t}E_\mathrm{b} = -P_\mathrm{int}.
	\end{equation}
\end{small}%
\endgroup


\subsection{Performance Requirements}\label{sec:methodology_performance}
In this section, we derive the performance requirements of the vehicle in order to ascertain that the gradeability, top speed, and acceleration are within acceptable limits. In line with~\cite{VerbruggenSalazarEtAl2019}, we capture the gradeability requirement as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		m_\mathrm{v}  \cdot g \cdot \sin{(\alpha_\mathrm{start})} \cdot r_\mathrm{w} \leq T_\mathrm{m,max} \cdot \eta_\mathrm{fd} \cdot \gamma_{\mathrm{fd}} \left\{\begin{array}{ll}
			\eta_\mathrm{fgt} \cdot \gamma_1 & \text{ if FGT } \\ 
			\eta_\mathrm{cvt} \cdot \gamma_\mathrm{max} & \text{ if CVT},
		\end{array}\right.
		\label{eq:SlopeStartConstraint}
	\end{equation}
\end{small}%
\endgroup
where $\alpha_\mathrm{start}$ is the required starting gradient. Furthermore, we include the following constraint from the extended version of~\cite{KorziliusBorsboomEtAl2021} to satisfy the acceleration requirement
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
		\frac{r_\mathrm{w} \cdot \omega_\mathrm{m,b}}
		     {\sqrt{\frac{2 \cdot P_\mathrm{m,max} \cdot \eta_\mathrm{gb} \cdot \eta_\mathrm{fd} \cdot t_\mathrm{acc}}{m_\mathrm{v}} - v_\mathrm{acc}^2} }
   		\leq
   		\begin{cases}
   			\gamma_\mathrm{fgt} &\text{ if FGT},   \\
   			\gamma_\mathrm{max} & \text{ if CVT},  
   		\end{cases}
		\label{eq:AccelerationConstraint}
	\end{equation}
\end{small}%
\endgroup
where $\omega_\mathrm{m,b}$ is the base speed of the vehicle and is a known parameter, $\eta_\mathrm{gb} = \eta_\mathrm{fgt}$ and $\eta_\mathrm{gb} = \eta_\mathrm{cvt}$ are efficiencies of FGT and CVT, respectively. Lastly, in line with~\cite{KorziliusBorsboomEtAl2021}, we ensure that the EM can deliver the required torque to propel the vehicle at its top speed on a flat road using the constraint
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks
\begin{small}
	\begin{equation}
%		P_{\mathrm{v,max}} \leq d_\mathrm{1,min} \cdot \omega_{\mathrm{m}} + d_\mathrm{0,min}
		\label{eq:TopSpeedConstraint}
			\begin{aligned}[b]
			T_\mathrm{req}(v_\mathrm{max}) \leq \min(&T_\mathrm{em,max}\cdot \eta_\mathrm{fd}\cdot \eta_\mathrm{gb}\cdot \gamma_\mathrm{x}\cdot \gamma_\mathrm{fd}, \\
			& (d_\mathrm{1,max}\cdot\gamma_\mathrm{x}\cdot \gamma_\mathrm{fd}~+d_\mathrm{0,max}\cdot \frac{r_\mathrm{w}}{v_\mathrm{max}})\cdot \eta_\mathrm{fd}\cdot\eta_\mathrm{gb}),
		\end{aligned}
	\end{equation}
\end{small}%
\endgroup
%where $P_{\mathrm{v,max}}$ is the power required at the vehicle's top speed, $v_\mathrm{max}$, and can be computed as
where $\gamma_{\mathrm{x}} = \gamma_{\mathrm{fgt}}$ for the FGT, $\gamma_{\mathrm{x}} = \gamma_{\mathrm{min}}$ for the CVT, $T_\mathrm{req}(v_\mathrm{max})$ is the torque required at the vehicle's top speed, $v_\mathrm{max}$, and can be computed as
\par\nobreak\vspace{-5pt}
\begingroup
\allowdisplaybreaks 
\begin{small}
	\begin{equation}
		\label{eq:Power_vmax}
		T_\mathrm{req}(v_\mathrm{max}) = \frac{P_\mathrm{req}(v_\mathrm{max},0,0)}{v_\mathrm{max}} \cdot r_\mathrm{w}.
%			P_{\mathrm{v,max}} =  \frac{1}{2} \cdot \rho_{\mathrm{a}} \cdot c_{\mathrm{d}} \cdot A_{\mathrm{f}} \cdot v_\mathrm{max}^3 + m_\mathrm{v}  \cdot g \cdot c_{\mathrm{r}} \cdot v_\mathrm{max},
	\end{equation}
\end{small}%
\endgroup


\subsection{Optimization Problem}\label{sec:methodology_optimization_problem}
Below we present a two-step algorithm based on convex optimization to solve the optimal control problem. The state variables for both the transmission technologies are $x = (E_\mathrm{b},\vartheta_{\mathrm{sft}},\vartheta_{\mathrm{rtr}},\vartheta_{\mathrm{mgt}},\vartheta_{\mathrm{str}},\vartheta_{\mathrm{wdg}},\vartheta_{\mathrm{ewdg}})$. The control and design varibles for FGT are $u = P_\mathrm{brk}$ and $p_\mathrm{FGT} = \gamma_\mathrm{fgt}$, respectively. The control variables for CVT are $u = (P_\mathrm{brk},\gamma(t))$. 
%Additionally, due to the nonlinear nature of Problem~\ref{prob:NLP}, the convergence is highly dependent on the initial conditions. 
Albeit the Problem~\ref{prob:NLP} is convex, it does not converge without a warm-start. In order to promote convergence, we present the two-step Algorithm~\ref{alg:algorithm} based on the following problems:
\begin{prob}[Nonlinear Convex Problem]\label{prob:NLP}
	The minimum-energy control strategies for the state-of-the-art EM loss models and energy-dependent battery model are the solution to the following nonlinear programming (NLP) problem:
	\par\nobreak\vspace{-5pt}
	\begingroup
	\allowdisplaybreaks
	\begin{small}
		\begin{equation*}
			\begin{aligned}
				\min~~&\Delta E_\mathrm{b} = E_{\mathrm{b}}(0) - E_{\mathrm{b}}(\mathrm{T})\\
				\text{s.t. }&\eqref{eq:Power_Balance_FD}-\eqref{eq:Shaft_Losses}, \eqref{eq:Rtr_Loss_Complex}-\eqref{eq:INV_BAT_AUX_Equillibrium},\eqref{eq:BAT_INT_Losses_Complex}-\eqref{eq:Power_vmax}.
			\end{aligned}
		\end{equation*}
	\end{small}%
	\endgroup
\end{prob}
\begin{prob}[Simplified Convex Problem]\label{prob:QCQP}
	The minimum-energy control strategies for the temperature-independent EM loss models and energy-independent battery model are the solution of the following quadratically constrained quadratic programming (QCQP) problem:
	\par\nobreak\vspace{-5pt}
	\begingroup
	\allowdisplaybreaks
	\begin{small}
		\begin{equation*}
			\begin{aligned}
				\min~~&\Delta E_\mathrm{b} = E_{\mathrm{b}}(0) - E_{\mathrm{b}}(\mathrm{T})\\
				\text{s.t. }&\eqref{eq:Power_Balance_FD}-\eqref{eq:EM_loss_simple1}, \eqref{eq:MOT_Torque_Limit}-\eqref{eq:BAT_INT_Losses},\eqref{eq:BAT_SOC_Limit}-\eqref{eq:Power_vmax}.
			\end{aligned}
		\end{equation*}
	\end{small}%
	\endgroup
\end{prob}
Since the KKT point of Problem~\ref{prob:QCQP} is globally optimal, Algorithm~\ref{alg:algorithm} leverages the solution generated by Problem~\ref{prob:QCQP} to warm-start Problem~\ref{prob:NLP}, thereby accelerating convergence and reducing computation time.
\begin{algorithm}[t!]
	\caption{: Two-step Optimization Algorithm}
	\label{alg:algorithm}
	\begin{algorithmic}
%		\State Given Motor:
		\State $\hat{E}_\mathrm{b}$ $\leftarrow$ Solve Problem~\ref{prob:QCQP}
		\State Initial Guess: ${E}_\mathrm{b}^\star = \hat{E}_\mathrm{b}$
		\State Precompute $a_\mathrm{rtr}$, $a_\mathrm{str}$, $a_\mathrm{mgt}$, $a_\mathrm{wdg}$, $R_\mathrm{mgt}$, $R_\mathrm{wdg}$
		\State ${E}_\mathrm{b}^\star$ $\leftarrow$ Solve Problem~\ref{prob:NLP}
%				\State Guess $\gamma_{\mathrm{guess}}>0}$
%		\State $\bar{v}(s)$ $\leftarrow$ Solve Problem~\ref{prob:SIM}%($\gamma_{\mathrm{guess}}(s)$)
%		\While{norm($v - \bar{v}$) $\geq \varepsilon_v$  }
%		\State  $\bar{v}(s) = v(s)$
%		\State  $v(s)$ $\leftarrow$ Solve Problem~\ref{prob:SDM}
%		\EndWhile
	\end{algorithmic}
\end{algorithm}

\subsection{Discussion}
A few comments are in order. 
%
First, in line with the current practices in high-level design and optimization of automotive powertrains~\cite{VerbruggenSalazarEtAl2019}, we assume constant efficiencies for the FGT, the CVT and neglect the dynamics of the CVT since the transmission modeling is not the aim of this thesis. We refer readers to~\cite{FahdzyanaSalazarEtAl},~\cite{FahdzyanaSalazarEtAl2021}, where a more careful analyses of the CVT dynamics are presented.
%
%Second, we exclude the gearbox and inverter temperatures because we lack data and high-fidelity models to validate our results.
Second, we exclude the gearbox, inverter temperatures from our LPTN and assume them not to be the limiting factors. However, they are crucial in designing the control strategies for a thermally constrained powertrain, and we can easily extend our framework to accommodate the temperatures. Interested readers are directed to~\cite{MK_WeiHofman2021CoDesign} for more information. 
%
Third, to minimize the propagation of error from loss models, we identify the LPTN for each driving cycle. This is because the LPTN is sensitive to error propagation, and a single node's error can spread to its neighbors. Furthermore, frequent under-estimation and over-estimation can result in diverging temperatures, putting accuracy at risk.
%
Fourth, we consider the average temperatures of each node during fitting and validation of the LPTN to preserve the physical meaning of the LPTN. However, the average temperatures can be replaced by hot-spot temperatures. We must note that this might be detrimental to the accuracy of the LPTN model. Moreover, we can lower the average temperature limits of each component in order to emulate the hot-spot temperature limits. 
%
Finally, we neglect the thermal dynamics of the coolant and assume it to be kept at a constant temperature, $\vartheta_{\mathrm{col}}$, by the radiator. Despite this assumption, our results in Section~\ref{sec:results} show that our models can accurately estimate the temperatures of each component of the EM.
%
%Finally, we cannot solve the problem using dedicated nonlinear solvers such as MOSEK



%\subsection{Notes}
%\mkmargin{We must note that the temperatures of transmission and inverter are not considered but their losses are. However, this is not entirely true. We must consider their temperatures in order to capture the effect more effectively. Furthermore, the effects of ram air are neglected because most of the latest EVs use louvers to close the front grill inorder to decrease aerodynamic drag. In which case the effect of ram air is none. Nonetheless, our approach is more robust because the fan can remove heat even when the ram air is zero (when the wind direction is in the direction of the evhicle)}{.}
%{Note: 1. The thermodynamic boundary conditions evolve much more slowly that, from an engine system point of view, these effects must be modelled as dynamic processes~\cite{MK_GuzzellaOnder2009Introduction}. 2. The average temperature of windings is considered. However, there is a difference between the temps of windings because all the windings are not active at the same time. This is neglected. 3. The hot spot temp and the end-winding temp are also neglected. 4. The effect of cold start on transmission oil temperature which leads to higher losses is also neglected in this research. 5. Should the effect of ram air on radiatoor be neglected? 6.The types of cooling (end-winding spray cooling, shaft hole cooling, air cooled motor,) is not considered. 7.The radiato desing (fin type, flow direction, core depth(dimensions) material, surface area to coolant ratio) is not considered. 8. The direction of wind for the ram air velocity is considered to be against the direction of motion of the vehicle. The effects of cross wind and tail wind are neglected. 9. The thermal conductivity of coolant is highly dependent on temperature which is ignored here. 10. The effect of cold-start (higher frictional losses due to lubricating oil viscosity) are neglected in this thesis. However, they can have significant effect on control strategy design as mentioned in \cite{MK_WeiHofman2019Energy}. 11. Most of the current generation cars have inverter, motor, transmission as a single unit. So, heat conduction is present between them as considered in \cite{WeiHofman2021CoDesign}. However, this is not considered in this case. 12.The radiator efficiency is a function of the air flow rate. however it is not considered here. 13. Assumption: No heat transfers occur in the system other than the ones mentioned in the above models. 14. The battery charging produces a lot of heat. However, we are not considering this phenomenon because it is a different circuit.}

